Exploiting Universal Redundancy

Fault tolerance is essential for building reliable services; however, it comes at the price of redundancy, mainly the "replication factor" and "diversity". With the increasing reliance on Internet-based services, more machines (mainly servers) are needed to scale out, multiplied with the extra expense of replication. This paper revisits the very fundamentals of fault tolerance and presents "artificial redundancy": a formal generalization of "exact copy" redundancy in which new sources of redundancy are exploited to build fault tolerant systems. On this concept, we show how to build "artificial replication" and design "artificial fault tolerance" (AFT). We discuss the properties of these new techniques showing that AFT extends current fault tolerant approaches to use other forms of redundancy aiming at reduced cost and high diversity.

==> _I.tex <==

%define theorems
\RequirePackage{amsthm}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem} % reset theorem numbering for each chapter

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition} % definition numbers are dependent on theorem numbers
\newtheorem{example}[theorem]{Example} % same for example numbers
\newtheorem{lemma}[theorem]{Lemma} % same for example numbers

%\providecommand{theorem}{Theorem}
%\providecommand{definition}{Definition}
%\providecommand{lemma}{Lemma}
%\providecommand{example}{Example}

%multirow table cell that accepts line breaks and 
%centers them by default, usage: 
% \mrcell{line1\\line2} or \mrcell[l]{leftline1\\leftline2}
\newcommand{\mrcellI}[2][c]{%
	\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}
	
%colored comments with yellow as default
\RequirePackage{xcolor}
\newcommand\noteI[2][yellow]{\colorbox{#1}{#2}}

% paragraph
\newcommand\parI[1]{\noindent \textbf{#1. }}


==> _II.tex <==
\RequirePackage{latexsym}
\RequirePackage{dsfont}

% macros for domain teory, semantics, etc. 

% math code definitions

%%%%%%%%%%%%%%%%%%%%%%%%\mathcode`:="603A          % : as punctuation
\mathcode`.="613A          % . as punctuation
\mathcode`|="326A          % | as a relation

\let\es=\relax    %  possible space before punctuation in displayed formulas

%% relations

\newcommand\tx[1]{\hbox{ #1 }}
\newcommand{\defeq}{\stackrel{.}{=}}

\let\vect=\overrightarrow
\let\iff=\Leftrightarrow        % this redefines the original
\let\implies=\Rightarrow
\let\implied=\Leftarrow

\let\sqleq=\sqsubseteq
\let\sqgeq=\sqsupseteq
\let\pleq=\sqleq          % partial-order leq
\let\pgeq=\sqgeq          % partial-order geq

\def\land{\mathrel{\wedge}}
\def\lor{\mathrel{\vee}}
\let\bigland=\bigwedge
\let\biglor=\bigvee

\def\preleq{\mathrel{%      % pre-order leq
  \raise 2pt\hbox{$\mathop\sqsubset\limits_{\hbox{$\sim$}}$}%
}}

% operators

\let\union=\cup
\let\bigunion=\bigcup
\let\join=\sqcup
\let\bigjoin=\bigsqcup
\let\meet=\sqcap
%\let\bigmeet=\bigsqcap
\newcommand{\down}{\mathord{\downarrow}}

\newcommand\setsize[1]{\left| #1 \right|}
\newcommand\domxtn{\mathbin{\stackrel{+}{|}}}
%\newcommand\domsub{\mathbin{\stackrel{-}{|}}}
\newcommand\domainsub{\mathop{\lhd\mkern-14mu-}}

% arrows

\newcommand{\map}{\mathrel{\hookrightarrow}}
\newcommand\goesto[1]{{\mathop{\longrightarrow}\limits^{#1}}}
\newcommand\goes{\longrightarrow}

% function constants

\newcommand\auxfun[1]{\expandafter\newcommand\csname #1\endcsname{%
 \mathop{\hbox{$\mathsf{#1}$}}\nolimits}}
 \newcommand\af[1]{\mathop{\hbox{$\mathsf{#1}$}}\nolimits}
 \newcommand\kw[1]{\mathrel{\hbox{$\mathbf{#1}$}}}

\auxfun{Max}
\auxfun{fix}
\auxfun{dom}
\auxfun{fst}
\auxfun{snd}
\auxfun{ran}

% sets

\newcommand{\pow}[1]{{\cal P}(#1)}
\newcommand{\bool}{\mathds{B}}
\newcommand{\nat}{\mathds{N}}
\newcommand{\ids}{\mathds{I}}



%%%%%%%%%%%

\newcommand\letin[2]{\mathop{\hbox{$\mathrm{let}$}} #1 \Leftarrow #2 . }
\newcommand\lift[1]{\lfloor #1 \rfloor}

\newcommand\true{\mathrm{true}}
\newcommand\false{\mathrm{false}}

%%%%%%%%%%%%%%%%%%%%%

\newcommand\iffdef{\mathrel{\Longleftrightarrow}}
\newcommand\nullstring{\epsilon}
\newcommand\pfunc{\hookrightarrow}
\newcommand\func{\rightarrow}


